Concise Plane Arrangements for Low-Poly Surface and Volume Modelling

Plane arrangements are a useful tool for surface and volume modelling. However, their main drawback is poor scalability. We introduce two key novelties that enable the construction of plane arrangements for complex objects and entire scenes: (i) an ordering scheme for the plane insertion and (ii) the direct use of input points during arrangement construction. Both ingredients reduce the number of unwanted splits, resulting in improved scalability of the construction mechanism by up to two orders of magnitude compared to existing algorithms. We further introduce a remeshing and simplification technique that allows us to extract low-polygon surface meshes and lightweight convex decompositions of volumes from the arrangement. We show that our approach leads to state-of-the-art results for the aforementioned tasks by comparing it to learning-based and traditional approaches on various different datasets. Our implementation is available at https://github.com/raphaelsulzer/compod .

==> figures/bspnet/bspnet_figure.tex <==
\begin{figure}
	\definetrim{mytrim1}{0 0 0 0}
	\definetrim{mytrim2}{100 10 100 10}
	\definetrim{mytrim3}{100 50 100 50}
	\definetrim{mytrim4}{0 0 0 0}
	\newcommand{\mywidth}{0.33\columnwidth}
	\newcommand{\myfontsize}{\footnotesize}

\begin{tabular}{@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_compod.jpg}
\\
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_compod.jpg}
\\
\myfontsize Input & \myfontsize BSP-Net~\cite{chen2020bspnet} & \myfontsize Ours
\end{tabular}
 \vspace{\captionvertspace}
\caption{\textbf{Comparison on Volume Decomposition with Intersecting Convexes.}
BSP-Net produces highly overlapping convexes (see the z-fighting) and exhibits generalisation issues (see right armrest of the sofa). Our approach produces weakly overlapping convexes that more accurately capture the fine components of the models. Note, how each pillow is described by a single convex.}
\label{fig:bspnet}
\end{figure}


==> figures/coacd/coacd_figure.tex <==
\begin{figure}[ht]
	\definetrim{temple}{80 0 130 0}
	\definetrim{templeclose}{230 20 200 310}
	\newcommand{\temple}{0.33\columnwidth}
	\definetrim{droid}{0 0 10 0}
	\definetrim{droidclose}{0 250 450 550}
	\newcommand{\droid}{0.33\columnwidth}

\begin{tabular}{@{}c@{}c@{}c@{}}
% Droid
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_mesh.pdf}
% \put(10,600){\color{black}\linethickness{0.1mm}%
% \frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_mesh.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_coacd.pdf}
\put(10,600){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_0.017_coacd_edges.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_compod.pdf}
\put(10,600){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_300_compod_edges.jpg}}}
\end{overpic}
\\
% Temple
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_mesh.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_mesh_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_0.015_coacd.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_0.015_coacd_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_10k_compod.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_10k_compod_close.jpg}}}
\end{overpic}
\\
Input & CoACD~\cite{wei2022coacd} & Ours
\end{tabular}
 \vspace{\captionvertspace}
\caption{\textbf{Comparison on volume decomposition with intersection-free convexes:}
The top row shows two decompositions for both methods of the \emph{Droid} with different levels of complexity. The bottom row shows a decomposition of the \emph{Temple} for both methods.
For a similar number of convexes (colored cells), our algorithm captures the geometry better (see stairs on the bottom close-up), with fewer facets (see edges on the top close up).}
% We compare our volume decompositions to the ones of CoACD~\cite{wei2022coacd}.}
\label{fig:coacd}
\end{figure}


==> figures/coacd/coacd_plot.tex <==
\begin{figure}
\includegraphics[width=\columnwidth,trim=18 0 42 20,clip]{figures/coacd/all.png}
\vspace{\captionvertspace}
\caption{\textbf{Quantitative comparison on volume decomposition with intersection-free convexes.} 
The volumetric IoU in function of the number of cells $|C_V|$ and facets $|F_V|$.
Our algorithm offers a similar trade-off between IoU and number of convexes than CoACD \cite{wei2022coacd}, but with convexes with fewer facets.}
% We compare our volume decompositions to the ones of CoACD~\cite{wei2022coacd}. Here, we show the volumetric IoU in function of the number of cells $|C_V|$ and facets $|F_V|$.}

\label{fig:coacd_plot}
\end{figure}


==> figures/pipeline/pipeline_figure.tex <==
\begin{figure*}[t]
\captionsetup[figure]{position=auto}
\newcommand{\mywidth}{0.19\linewidth}
\newcommand{\mywidthd}{0.38\linewidth}
\definetrim{mytrim}{90 120 110 120}
\definetrim{mytrimd}{20 70 40 70}

\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
\centering
\begin{subfigure}{\mywidth}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/1.png}
\vspace{-1.5\baselineskip}
\caption{Point cloud}
\label{subfig:pipeline_a}
\end{subfigure}
&
\multicolumn{2}{c}{
\multirow{2}{*}[7.1em]{
\begin{subfigure}{\mywidthd}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrimd]{figures/pipeline/steps/3.png}
\vspace{-1.5\baselineskip}
\caption{Compact plane arrangement}
\label{subfig:pipeline_c}
\end{subfigure}
}}
&
\begin{subfigure}{\mywidth}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/5.png}
\vspace{-2\baselineskip}
\caption{Surface mesh}
\label{subfig:pipeline_d}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/6.png}
\vspace{-2\baselineskip}
\caption{\emph{remeshed}}
\label{subfig:pipeline_f}
\end{subfigure}
\\
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{-5}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/2.png}
\vspace{-1.5\baselineskip}
\caption{Planes with inlier points}
\label{subfig:pipeline_b}
\end{subfigure}
&
&
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{2}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/7.png}
\vspace{-2\baselineskip}
\caption{Volume mesh}
\label{subfig:pipeline_e}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/8.png}
\vspace{-2\baselineskip}
\caption{\emph{simplified}}
\label{subfig:pipeline_g}
\end{subfigure}


\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Pipeline.}
Our method processes a set of planes with their corresponding inlier points \subref{subfig:pipeline_b} detected from a point cloud \subref{subfig:pipeline_a} into a compact plane arrangement \subref{subfig:pipeline_c}. From this arrangement we extract either a watertight and intersection-free surface mesh \subref{subfig:pipeline_d} or a volume mesh with intersection-free convexes \subref{subfig:pipeline_e}.
The surface mesh can optionally be remeshed to represent each planar region with only one facet,
and with Delaunay triangles for regions with holes \subref{subfig:pipeline_f}. The remeshed surface is still watertight and intersection-free.
The volume mesh can be simplified by merging groups of convex volumes and potentially allowing them to overlap \subref{subfig:pipeline_g}.}
\label{fig:pipeline}
\end{figure*}


==> figures/robust/robust_figure.tex <==
\begin{figure}
	\definetrim{mytrim1}{0 0 0 0}
	\definetrim{mytrim2}{100 10 100 10}
	\definetrim{mytrim3}{100 50 100 50}
	\definetrim{mytrim4}{0 0 0 0}
	\newcommand{\mywidth}{0.32\columnwidth}

\begin{tabular}{@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_robust_edges.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_compod_edges.jpg}
\\
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_robust_edges.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_compod_edges.jpg}
\\
Input&RLPM~\cite{chen2023robust} & Ours
\end{tabular}
 \vspace{-2mm}
\caption{\textbf{Comparison on surface mesh simplification.} RLPM preserves sharp features but not small details. Our method reconstructs meshes with fewer facets while preserving small details such as the teeth (top row) or the bricks (bottom row).}
\label{fig:robust}
\end{figure}


==> figures_backup/bspnet/bspnet_figure.tex <==
\begin{figure}
	\definetrim{mytrim1}{0 0 0 0}
	\definetrim{mytrim2}{100 10 100 10}
	\definetrim{mytrim3}{100 50 100 50}
	\definetrim{mytrim4}{0 0 0 0}
	\newcommand{\mywidth}{0.33\columnwidth}
	\newcommand{\myfontsize}{\footnotesize}

\begin{tabular}{@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_compod.jpg}
\\
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_compod.jpg}
\\
\myfontsize Input & \myfontsize BSP-Net~\cite{chen2020bspnet} & \myfontsize Ours
\end{tabular}
 \vspace{\captionvertspace}
\caption{\textbf{Comparison on Volume Decomposition with Intersecting Convexes.}
BSP-Net produces highly overlapping convexes (see the z-fighting) and exhibits generalisation issues (see right armrest of the sofa). Our approach produces weakly overlapping convexes that more accurately capture the fine components of the models. Note, how each pillow is described by a single convex.}
\label{fig:bspnet}
\end{figure}


==> figures_backup/bspnet/combined_eccv/combined.tex <==
\begin{figure}
    
\begin{tabular}{@{}cc@{}}

\begin{subfigure}{0.28\linewidth}
    \input{figures/bspnet/combined_eccv/table.tex}
    \caption{Quantitative}
\end{subfigure}
&
\begin{subfigure}{0.72\linewidth}
    \input{figures/bspnet/combined_eccv/figure.tex}
    \caption{Qualitative}
\end{subfigure}


\end{tabular}
\caption{\textbf{Comparison on Volume Decomposition with Intersecting Convexes.} %Our algorithm compared to the learned convex decomposition of BSP-Net~\cite{chen2020bspnet} on their dataset (ShapeNet). 
%BSP-Net inputs a voxel grid of $64^3$ while we input 100\,000 points together with detected planes. 
BSP-Net produces highly overlapping convexes (see the z-fighting) and exhibits generalisation issues (see right armrest of the sofa). Our approach produces weakly overlapping convexes that more accurately capture the fine components of the models. Note, how each pillow is described by a single convex.}
\label{fig:bspnet}
\end{figure}

==> figures_backup/bspnet/combined_eccv/figure.tex <==
\definetrim{mytrim1}{0 0 0 0}
\definetrim{mytrim2}{100 10 100 10}
\definetrim{mytrim3}{100 50 100 50}
\definetrim{mytrim4}{0 0 0 0}
\newcommand{\mywidth}{0.33\columnwidth}
\begin{tabular}{@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/04256520_d1f68ceddaa3b0bcfebad4f49b26ec52_compod.jpg}
\\
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_bspnet.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/bspnet/02958343_cbd0b4a0d264c856f35cb5c94d4343bf_compod.jpg}
\\
Input &BSP-Net~\cite{chen2020bspnet} & Ours
\end{tabular}


==> figures_backup/bspnet/combined_eccv/table.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}}
    \setlength{\tabcolsep}{7pt}
\begin{tabular}{@{}lrr}
    \toprule
    & \multicolumn{2}{c}{\emph{Complexity}}  \\
    \midrule
    & $|C_V|$ & $|F_V|$  \\
     &  &  \\
    \midrule
    \textbf{BSP-Net~\cite{chen2020bspnet}}  & 60.9 & 1646   \\
    \textbf{Ours}   & \bf 41.7  & \bf 773   \\
    \bottomrule
\end{tabular}
\\[1.5cm]
\setlength{\tabcolsep}{9pt}
\begin{tabular}{rr@{}}
    \toprule
    \multicolumn{2}{c}{\emph{Accuracy}}  \\
    \midrule
    \chamfersq~$\downarrow$ & \normal~$\uparrow$ \\
    ($\times 10^{3}$) &   \\
    \midrule
    0.771 & 0.817   \\
    \bf 0.385  & \bf 0.919  \\
    \bottomrule
\end{tabular}
\end{tabular}}


==> figures_backup/coacd/coacd_combined_eccv.tex <==
\begin{figure}[ht]
    \begin{tabular}{@{}cc@{}}
        \centering
        \begin{subfigure}{0.25\linewidth}
            \includegraphics[width=\linewidth,trim=18 0 2 10,clip]{figures/coacd/cells.png}
            % \vspace{-1.5\baselineskip}
        \caption{Cells}
        \label{subfig:coacd_a}
        \end{subfigure}
        &
        \multirow[vpos]{2}{*}{
        \centering
        \begin{subfigure}{0.74\linewidth}
            \addtocounter{subfigure}{1}
            \vspace{-8\baselineskip}
            \input{figures/coacd/coacd_figure_eccv}
        \caption{Qualitative}
        \label{subfig:coacd_c}
        \end{subfigure}}
        \\
        \begin{subfigure}{0.25\linewidth}
            \addtocounter{subfigure}{-2}
            \includegraphics[width=\linewidth,trim=18 0 2 10,clip]{figures/coacd/facets.png}
        \caption{Facets}
        \label{subfig:coacd_b}
        \end{subfigure}
    \end{tabular}
    \vspace{\captionvertspace}
    \caption{\textbf{Volume Decomposition with Non-Overlapping Convexes.} 
    We plot the volumetric IoU in function of the number of cells $|C_V|$ \Subref{subfig:coacd_a} and facets $|F_V|$ \Subref{subfig:coacd_b}.
    Our algorithm offers a trade-off between IoU and number of convexes similar to the one of CoACD \cite{wei2022coacd}, but with convexes with fewer facets.
    In \Subref{subfig:coacd_c}, the top row shows two decompositions for both methods of the \emph{Droid} with different levels of complexity. The bottom row shows a decomposition of the \emph{Temple}.
For a similar number of convexes (colored cells), our algorithm captures the geometry better (see stairs on the bottom close-up), with fewer facets (see edges on the top close up).}
\label{fig:coacd}
\end{figure}


==> figures_backup/coacd/coacd_figure.tex <==
\begin{figure}[ht]
	\definetrim{temple}{80 0 130 0}
	\definetrim{templeclose}{230 20 200 310}
	\newcommand{\temple}{0.33\columnwidth}
	\definetrim{droid}{0 0 10 0}
	\definetrim{droidclose}{0 250 450 550}
	\newcommand{\droid}{0.33\columnwidth}

\begin{tabular}{@{}c@{}c@{}c@{}}
% Droid
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_mesh.pdf}
% \put(10,600){\color{black}\linethickness{0.1mm}%
% \frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_mesh.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_coacd.pdf}
\put(10,600){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_0.017_coacd_edges.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_compod.pdf}
\put(10,600){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_300_compod_edges.jpg}}}
\end{overpic}
\\
% Temple
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_mesh.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_mesh_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_0.015_coacd.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_0.015_coacd_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_10k_compod.jpg}
\put(600,0){\color{black}\linethickness{0.1mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_10k_compod_close.jpg}}}
\end{overpic}
\\
Input & CoACD~\cite{wei2022coacd} & Ours
\end{tabular}
 \vspace{\captionvertspace}
\caption{\textbf{Comparison on volume decomposition with intersection-free convexes:}
The top row shows two decompositions for both methods of the \emph{Droid} with different levels of complexity. The bottom row shows a decomposition of the \emph{Temple} for both methods.
For a similar number of convexes (colored cells), our algorithm captures the geometry better (see stairs on the bottom close-up), with fewer facets (see edges on the top close up).}
% We compare our volume decompositions to the ones of CoACD~\cite{wei2022coacd}.}
\label{fig:coacd}
\end{figure}


==> figures_backup/coacd/coacd_figure_eccv.tex <==
\definetrim{temple}{80 0 130 0}
\definetrim{templeclose}{230 20 200 310}
\newcommand{\temple}{0.33\columnwidth}
\definetrim{droid}{0 0 10 0}
\definetrim{droidclose}{0 250 450 550}
\newcommand{\droid}{0.33\columnwidth}
\newcommand{\myfontsize}{\footnotesize}
\begin{tabular}{@{}c@{}c@{}c@{}}
% Droid
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_mesh.pdf}
% \put(10,600){\color{yellow}\linethickness{0.35mm}%
% \frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_mesh.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_coacd.pdf}
\put(30,600){\color{yellow}\linethickness{0.35mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_0.017_coacd_edges.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\droid,droid]
{figures/coacd/images/droid_compod.pdf}
\put(30,600){\color{yellow}\linethickness{0.35mm}%
\frame{\includegraphics[scale=.06,droidclose]{figures/coacd/images/droid_300_compod_edges.jpg}}}
\end{overpic}
\\
% Temple
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_mesh.jpg}
\put(600,0){\color{yellow}\linethickness{0.35mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_mesh_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_0.015_coacd.jpg}
\put(600,0){\color{yellow}\linethickness{0.35mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_0.015_coacd_close.jpg}}}
\end{overpic}
&
\begin{overpic}[width=\temple,temple]
{figures/coacd/images/temple_10k_compod.jpg}
\put(600,0){\color{yellow}\linethickness{0.35mm}%
\frame{\includegraphics[scale=.045,templeclose]{figures/coacd/images/temple_10k_compod_close.jpg}}}
\end{overpic}
\\
\myfontsize Input & \myfontsize CoACD~\cite{wei2022coacd} & \myfontsize Ours
\end{tabular}

==> figures_backup/coacd/coacd_plot.tex <==
\begin{figure}
\includegraphics[width=\columnwidth,trim=18 0 42 20,clip]{figures/coacd/all.png}
\vspace{\captionvertspace}
\caption{\textbf{Quantitative comparison on volume decomposition with intersection-free convexes.} 
The volumetric IoU in function of the number of cells $|C_V|$ and facets $|F_V|$.
Our algorithm offers a similar trade-off between IoU and number of convexes than CoACD \cite{wei2022coacd}, but with convexes with fewer facets.}
% We compare our volume decompositions to the ones of CoACD~\cite{wei2022coacd}. Here, we show the volumetric IoU in function of the number of cells $|C_V|$ and facets $|F_V|$.}

\label{fig:coacd_plot}
\end{figure}


==> figures_backup/pipeline/pipeline_figure.tex <==
\begin{figure*}[t]
\captionsetup[figure]{position=auto}
\newcommand{\mywidth}{0.19\linewidth}
\newcommand{\mywidthd}{0.38\linewidth}
\definetrim{mytrim}{90 120 110 120}
\definetrim{mytrimd}{20 70 40 70}

\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
\centering
\begin{subfigure}{\mywidth}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/1.png}
\vspace{-1.5\baselineskip}
\caption{Point cloud}
\label{subfig:pipeline_a}
\end{subfigure}
&
\multicolumn{2}{c}{
\multirow{2}{*}[7.1em]{
\begin{subfigure}{\mywidthd}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrimd]{figures/pipeline/steps/3.png}
\vspace{-1.5\baselineskip}
\caption{Compact plane arrangement}
\label{subfig:pipeline_c}
\end{subfigure}
}}
&
\begin{subfigure}{\mywidth}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/5.png}
\vspace{-2\baselineskip}
\caption{Surface mesh}
\label{subfig:pipeline_d}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/6.png}
\vspace{-2\baselineskip}
\caption{\emph{remeshed}}
\label{subfig:pipeline_f}
\end{subfigure}
\\
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{-5}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/2.png}
\vspace{-1.5\baselineskip}
\caption{Planes with inlier points}
\label{subfig:pipeline_b}
\end{subfigure}
&
&
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{2}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/7.png}
\vspace{-2\baselineskip}
\caption{Volume mesh}
\label{subfig:pipeline_e}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
\addtocounter{subfigure}{1}
\includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/8.png}
\vspace{-2\baselineskip}
\caption{\emph{simplified}}
\label{subfig:pipeline_g}
\end{subfigure}


\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Pipeline.}
Our method processes a set of planes with their corresponding inlier points \subref{subfig:pipeline_b} detected from a point cloud \subref{subfig:pipeline_a} into a compact plane arrangement \subref{subfig:pipeline_c}. From this arrangement we extract either a watertight and intersection-free surface mesh \subref{subfig:pipeline_d} or a volume mesh with intersection-free convexes \subref{subfig:pipeline_e}.
The surface mesh can optionally be remeshed to represent each planar region with only one facet,
and with Delaunay triangles for regions with holes \subref{subfig:pipeline_f}. The remeshed surface is still watertight and intersection-free.
The volume mesh can be simplified by merging groups of convex volumes and potentially allowing them to overlap \subref{subfig:pipeline_g}.}
\label{fig:pipeline}
\end{figure*}


==> figures_backup/pipeline/pipeline_figure_eccv.tex <==
\begin{figure*}[t]
    \captionsetup[figure]{position=auto}
    \newcommand{\mywidth}{0.19\linewidth}
    \newcommand{\mywidthd}{0.38\linewidth}
    \definetrim{mytrim}{90 120 110 120}
    \definetrim{mytrimd}{20 70 40 70}
    
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
    \centering
    \begin{subfigure}{\mywidth}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/1.jpg}
    \vspace{-1.5\baselineskip}
    \caption{Point cloud}
    \label{subfig:pipeline_a}
    \end{subfigure}
    &
    \multicolumn{2}{c}{
    \multirow{2}{*}[5em]{
    \begin{subfigure}{\mywidthd}
    \addtocounter{subfigure}{1}
    \includegraphics[width=\linewidth,mytrimd]{figures/pipeline/steps/3.jpg}
    \vspace{-1.5\baselineskip}
    \caption{Compact plane arrangement}
    \label{subfig:pipeline_c}
    \end{subfigure}
    }}
    &
    \begin{subfigure}{\mywidth}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/5.jpg}
    \vspace{-1.5\baselineskip}
    \caption{Surface mesh}
    \label{subfig:pipeline_d}
    \end{subfigure}
    &
    \begin{subfigure}{\mywidth}
    \addtocounter{subfigure}{1}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/6.jpg}
    \vspace{-1.5\baselineskip}
    \caption{\emph{remeshed}}
    \label{subfig:pipeline_f}
    \end{subfigure}
    \\
    \begin{subfigure}{\mywidth}
    \addtocounter{subfigure}{-5}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/2.jpg}
    \vspace{-1.5\baselineskip}
    \caption{Planes}
    \label{subfig:pipeline_b}
    \end{subfigure}
    &
    &
    &
    \begin{subfigure}{\mywidth}
    \addtocounter{subfigure}{2}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/7.jpg}
    \vspace{-1.5\baselineskip}
    \caption{Volume mesh}
    \label{subfig:pipeline_e}
    \end{subfigure}
    &
    \begin{subfigure}{\mywidth}
    \addtocounter{subfigure}{1}
    \includegraphics[width=\linewidth,mytrim]{figures/pipeline/steps/8.jpg}
    \vspace{-1.5\baselineskip}
    \caption{\emph{simplified}}
    \label{subfig:pipeline_g}
    \end{subfigure}
    
    
    \end{tabular}
    \vspace{\captionvertspace}
    \caption{\textbf{Pipeline.}
    Our method processes a set of planes with their corresponding inlier points \Subref{subfig:pipeline_b} detected from a point cloud \Subref{subfig:pipeline_a} into a compact plane arrangement \Subref{subfig:pipeline_c}. From this arrangement we extract either a watertight and intersection-free surface mesh \Subref{subfig:pipeline_d} or a volume mesh with intersection-free convexes \Subref{subfig:pipeline_e}.
    The surface mesh can optionally be remeshed to represent each planar region with only one facet,
    and with Delaunay triangles for regions with holes \Subref{subfig:pipeline_f}. The remeshed surface is still watertight and intersection-free.
    The volume mesh can be simplified by merging groups of convex volumes and potentially allowing them to intersect \Subref{subfig:pipeline_g}.}
    \vspace{\captionpostvertspace}
    \label{fig:pipeline}
    \end{figure*}
    

==> figures_backup/robust/combined_eccv/combined.tex <==
\begin{figure}
    
\begin{tabular}{@{}cc@{}}

\begin{subfigure}{0.28\linewidth}
    \input{figures/robust/combined_eccv/table.tex}
    \caption{Quantitative}
    \label{subfig:robust_a}
\end{subfigure}
&
\begin{subfigure}{0.7\linewidth}
    \input{figures/robust/combined_eccv/figure.tex}
    \caption{Qualitative}
    \label{subfig:robust_b}
\end{subfigure}
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Surface Mesh Simplification.} We compare RLPM and our pipeline on models from Thingi10k. 
% Because RLPM produces triangle meshes and our method produces polygon meshes 
We triangulate our output and perform edge collapse based on QEM s.t. OursTri and RLPM have the same number of triangles. \Subref{subfig:robust_a} The runtimes of the methods, number of vertices $|V_S|$ and facets $|F_S|$ of the surface meshes (\ie triangles for RLPM and OursTri, and polygons for Ours), and Chamfer (CD) and Hausdorff distance (HD) and normal consistency (NC) between ground truth and reconstruction. \Subref{subfig:robust_b} The reconstructions of the \emph{Tower of Pi} from the dataset. Note how both, our polygon and our triangle mesh is much more detailed compare to the one of RLPM. 
% The meshes of OursTri and RLPM have the same number of triangles.
}
\label{fig:robust}
\end{figure}

==> figures_backup/robust/combined_eccv/figure.tex <==
\definetrim{mytrim1}{50 10 50 0}
\newcommand{\mywidth}{0.25\columnwidth}
\newcommand{\mywidthd}{\columnwidth}
\newcommand{\myfontsize}{\footnotesize}

%%% tikz stuff
\tikzstyle{closeup} = [
    opacity=1.0,          % opacity of both windows
    height=0.9cm,         %  height of large window
    width=0.9cm,          %   width of large window
    magnification=2.5,
    connect spies, yellow  % connects big and small window by a line
  ]
  \tikzstyle{largewindow} = [circle, yellow, line width=0.35mm]
  \tikzstyle{smallwindow} = [circle, yellow, line width=0.25mm]


\begin{tabular}{@{}c@{}c@{}c@{}c@{}}

\begin{subfigure}{\mywidth}
    \begin{tikzpicture}[spy using outlines={every spy on node/.append style={smallwindow}}]

      \coordinate (ai) at (-0.78,1.02);
      \coordinate (aj) at (0.5,1.6);

      \node[anchor=south] (FigA) at (0,0){%
      \includegraphics[width=\mywidthd,mytrim1]{figures/robust/87_gt.jpg}};
      \spy [closeup] on ($(FigA)+(ai)$) 
          in node[largewindow] at ($(FigA)+(aj)$);
    \end{tikzpicture}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
    \begin{tikzpicture}[spy using outlines={every spy on node/.append style={smallwindow}}]

      \node[anchor=south] (FigA) at (0,0){%
      \includegraphics[width=\mywidthd,mytrim1]{figures/robust/87_robust_edges.jpg}};
      \spy [closeup] on ($(FigA)+(ai)$) 
          in node[largewindow] at ($(FigA)+(aj)$);
    \end{tikzpicture}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
    \begin{tikzpicture}[spy using outlines={every spy on node/.append style={smallwindow}}]

      \node[anchor=south] (FigA) at (0,0){%
      \includegraphics[width=\mywidthd,mytrim1]{figures/robust/87_compod_edges.jpg}};
      \spy [closeup] on ($(FigA)+(ai)$) 
          in node[largewindow] at ($(FigA)+(aj)$);
    \end{tikzpicture}
\end{subfigure}
&
\begin{subfigure}{\mywidth}
    \begin{tikzpicture}[spy using outlines={every spy on node/.append style={smallwindow}}]

      \node[anchor=south] (FigA) at (0,0){%
      \includegraphics[width=\mywidthd,mytrim1]{figures/robust/87_compod_qed_edges.jpg}};
      \spy [closeup] on ($(FigA)+(ai)$) 
          in node[largewindow] at ($(FigA)+(aj)$);
    \end{tikzpicture}
\end{subfigure}
\vspace{\captionvertspace}
\\
\myfontsize Input& \myfontsize RLPM~\cite{chen2023robust} 
& \myfontsize Ours & \myfontsize OursTri
\end{tabular}

==> figures_backup/robust/combined_eccv/table.tex <==
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c@{}}
    \setlength{\tabcolsep}{7pt}
\begin{tabular}{@{}l@{}rrr}
    \toprule
    & \emph{Perform.} & \multicolumn{2}{c}{\emph{Complexity}}  \\
    \midrule
    & Time & $|V_S|$ & $|F_S|$  \\
    & (s) &  &  \\
    \midrule
    \textbf{RLPM~\cite{chen2023robust}} & 503 & 899 & 1969   \\
    \textbf{Ours} & \bf 410  & 2051 &  2045  \\
    \textbf{OursTri}  & 411 & \bf 879 & \bf 1936 \\
    \bottomrule
\end{tabular}
\\[1.5cm]
\setlength{\tabcolsep}{9pt}
\begin{tabular}{rrr@{}}
    \toprule
    \multicolumn{3}{c}{\emph{Accuracy}}  \\
    \midrule
    \chamfer~$\downarrow$ & \hausdorff~$\downarrow$ & \normal~$\uparrow$ \\
    ($\times 10^{2}$) & ($\times 10^{2}$)   \\
    \midrule
    0.269 & 2.48 & 0.923   \\
    \bf 0.218 &  \bf 2.10 & \bf 0.941  \\
     0.244 & 2.32 & 0.924  \\
    \bottomrule
\end{tabular}
\end{tabular}}

==> figures_backup/robust/robust_figure.tex <==
\begin{figure}
	\definetrim{mytrim1}{0 0 0 0}
	\definetrim{mytrim2}{100 10 100 10}
	\definetrim{mytrim3}{100 50 100 50}
	\definetrim{mytrim4}{0 0 0 0}
	\newcommand{\mywidth}{0.32\columnwidth}

\begin{tabular}{@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_robust_edges.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/4_compod_edges.jpg}
\\
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_gt.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_robust_edges.jpg}
&
\includegraphics[width=\mywidth,mytrim1]{figures/robust/7_compod_edges.jpg}
\\
Input&RLPM~\cite{chen2023robust} & Ours
\end{tabular}
 \vspace{-2mm}
\caption{\textbf{Comparison on surface mesh simplification.} RLPM preserves sharp features but not small details. Our method reconstructs meshes with fewer facets while preserving small details such as the teeth (top row) or the bricks (bottom row).}
\label{fig:robust}
\end{figure}


==> figures_backup/runtime/runtime_figure.tex <==
\begin{figure}[t]


%\subfloat[Runtime]{
    \centering
\includegraphics[width=0.7\columnwidth,trim=18 0 20 20,clip]{figures/runtime/graphs.png}

 \vspace{\captionvertspace}
\caption{\textbf{Scalability.} Average runtime (left) and memory peak (right) in function of the number of input planar shapes for different construction mechanisms. The transparent band around each curve indicates the minimal and maximal values measured on various models. Our algorithm offers the best performance and can process 10k planar shapes in around 30 minutes without exceeding the memory consumption of a standard computer. It also exhibits a better stability than other methods whose variation bands are thicker.}
% 40 to 500 is run on cpu
% 2000 and 10000 is run on gpu
\label{fig:runtime}

\end{figure}


==> figures_backup/teaser/teaser_figure.tex <==
\begin{figure}
% \vspace{-12pt}
\centering
% \includegraphics[width=\textwidth,trim=0 5 0 0, clip]{figures/teaser2/compod_teaser.pdf}
\includegraphics[width=\textwidth,trim=0 0 0 0, clip]{figures/teaser/teaser.jpg}
\vspace{\captionvertspace}
\caption{Our representation of the Meeting Room~\cite{tanksandtemples} as a watertight and intersection-free surface mesh with 90k polygonal facets (center) or as a simplified volume mesh with 2500 convex polyhedra (right). Our method inputs 40k planes (middle left) detected from a LiDAR scan of the scene (top left). For comparison, a Screened Poisson \cite{screened_poisson} reconstruction consists of over 6M triangles (bottom left).}
\vspace{\captionpostvertspace}
\label{fig:teaser}
\end{figure}


==> figures_backup/thingi/thingi_figure.tex <==
\begin{figure}[t]
\newcommand{\myfontsize}{\footnotesize}
	\definetrim{mytrim1}{150 110 150 150}
	\definetrim{mytrim2}{80 20 120 90}
	\definetrim{mytrim3}{100 50 100 50}
	\newcommand{\mywidth}{0.20\columnwidth}
	\newcommand{\mywidtht}{0.20\columnwidth}
\centering
% \begin{tabular}{@{}c@{}c@{}c@{}}
% \includegraphics[width=\mywidth,mytrim1]{figures/thingi/pointcloud.jpg}
% &
% \includegraphics[width=\mywidth,mytrim1]{figures/thingi/planes.jpg}
% &
% \includegraphics[width=\mywidth,mytrim1]{figures/thingi/mesh.jpg}
% \\
% Point cloud & Planes &
% Dense mesh
% \end{tabular}
\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/pointcloud.jpg}
&
\includegraphics[width=\mywidtht,mytrim2]{figures/thingi/exhaustive_partition.jpg}
&
\includegraphics[width=\mywidtht,mytrim2]{figures/thingi/abspy_partition.jpg}
&
\includegraphics[width=\mywidtht,mytrim2]{figures/thingi/ksr_partition.jpg}
&
\includegraphics[width=\mywidtht,mytrim2]{figures/thingi/ours_partition.jpg}
\\
\multicolumn{5}{l}{\vspace{-0.5cm}\myfontsize Point cloud}
\\
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/planes.jpg}
&
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/exhaustive_surface.jpg}
&
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/abspy_surface.jpg}
&
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/ksr_surface.jpg}
&
\includegraphics[width=\mywidtht,mytrim1]{figures/thingi/ours_surface.jpg}
\\
\myfontsize PC \& planes & \myfontsize Exhaustive~\cite{Edelsbrunner83} & \myfontsize Adaptive~\cite{Murali:1997:CSA} &  \myfontsize KSR~\cite{bauchet2020ksr} &   \myfontsize Ours
\end{tabular}
\vspace{\captionvertspace}
\caption{\textbf{Comparison with Plane Arrangements.}
Our algoritm builds a more concise plane arrangement than existing mechanisms (top row), leading to a polyon mesh with fewer facets (bottom row).
}
\label{fig:thingi}
\end{figure}


==> tables/bspnet.tex <==
\begin{table}
    \setlength{\tabcolsep}{12pt}
\centering
\caption{\textbf{Volume decomposition with intersecting convexes.}
The comparison is performed at a similar average number of convexes $|C_V|$. $|F_V|$ refers to the average number of facets in the output configuration of convexes.
% We compare our volume mesh reconstructions to the ones of BSP-Net~\cite{chen2020bspnet} on ShapeNet. $|C_V|$ is the number of cells and $|F_V|$ the number of facets of the reconstructed volume mesh. IoU is the volumetric intersection over union between reconstructed and ground truth mesh. Our reconstructions are much more accurate and more compact than the ones of BSP-Net~\cite{chen2020bspnet}.
}
\vspace{\captionvertspace}
\resizebox{0.7\columnwidth}{!}{%
%
%\begin{tabular}{@{}lrrr@{}HH@{}}
\begin{tabular}{lrrrrr}
\toprule
& \multicolumn{2}{c}{\emph{Complexity}} & \multicolumn{3}{c}{\emph{Accuracy}} \\
\midrule
& $|C_V|$ & $|F_V|$ & IoU & \chamfer & Hausdorff \\
\midrule
\textbf{BSP-Net~\cite{chen2020bspnet}} & 21.9 & 754 & 0.38 & 6.78 & 43.5  \\
\textbf{Ours} & \bf 19.6  & \bf 540 & \bf  0.90 & \bf 4.61 & \bf 42.9  \\
\bottomrule
\end{tabular}
}
\label{tab:bspnet}
\end{table}


==> tables/helsinki.tex <==
\begin{table}[t]
    \setlength{\tabcolsep}{12pt}
\centering
\caption{\textbf{Quantitative Comparison with Points2Poly~(P2P) on their Helsinki city dataset~\cite{chen2022points2poly}.}
We show the number of vertices $|V_S|$ and polygonal facets $|F_S|$ of building models. We also show the one-sided Hausdorff distance ($\text{\hausdorff}^{r\rightarrow g}$) measured from reconstructed to ground truth building models, the inverse distance ($\text{\hausdorff}^{g\rightarrow r}$), and the maximum of the two distances (\hausdorff). These values were computed using the evaluation pipeline provided by the authors of P2P. All metrics are computed as the mean value of the 45 building models.
Note, that some of the ground truth models contain interior structures which cannot be reconstructed due to missing input data. This corrupts the one-sided Hausdorff distance measured from ground truth models to reconstructions ($\text{\hausdorff}^{g\rightarrow r}$).
In the last column, we show the average reconstruction time per building.
}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
 & \multicolumn{2}{c}{\emph{Complexity}} & \multicolumn{3}{c}{\emph{Accuracy}} & \emph{Performance} \\
\midrule
 & $|V_S|$  & $|F_S|$  & $\text{\hausdorff}^{r\rightarrow g}$ & $\text{\hausdorff}^{g\rightarrow r}$	&  \hausdorff   & Time     \\
 &  & & $(\times 10^{2})$ & $(\times 10^{2})$ & $(\times 10^{2})$  & (s) \\
\midrule
\textbf{P2P}\cite{chen2022points2poly}& 419 &  103   &   4.71 & \bf  7.51     &     8.64 & 4.14     \\
\textbf{Adaptive} &      148  & 131 &       4.27 &    7.62    &    8.62 & 3.32     \\
\textbf{Ours} &  \bf  57.6 & \bf 41.2  &  \bf  3.30  &   7.65  & \bf 7.79 & \bf 2.60 \\
\bottomrule
\end{tabular}
}
\label{tab:p2p}
\end{table}

==> tables/robust.tex <==
\begin{table}
    \setlength{\tabcolsep}{12pt}
\centering
\caption{\textbf{Surface Mesh Simplification.}
%We compare our surface reconstruction pipeline to the mesh simplification of \acf{rlpm}~\cite{chen2023robust} on their Thingi10K subset.
Chamfer and Hausdorff are symmetric distances between input and output meshes.
Time is the runtime of the entire pipelines.
}
\vspace{\captionvertspace}
\resizebox{0.7\linewidth}{!}{%
%
\begin{tabular}{@{}lrrrrr@{}}
\toprule
& \multicolumn{2}{c}{\emph{Complexity}} & \multicolumn{2}{c}{\emph{Accuracy}} & \emph{Performance} \\
\midrule
& $|V_S|$ & $|F_S|$ & \chamfer & \hausdorff  & Time  \\
&  & & ($\times 10^{2}$) & ($\times 10^{2}$)  & (s) \\
\midrule
\textbf{RLPM~\cite{chen2023robust}} & 2019& 2019 & 0.280 & 2.69 & 503  \\
\textbf{Ours} & \bf 1232 & \bf 1232 & \bf 0.213 & \bf 1.84 & \bf 410 \\
\bottomrule
\end{tabular}
}
\label{tab:robust}
\end{table}

